Parallel $k$-Core Decomposition: Theory and Practice

This paper proposes efficient solutions for $k$-core decomposition with high parallelism. The problem of $k$-core decomposition is fundamental in graph analysis and has applications across various domains. However, existing algorithms face significant challenges in achieving work-efficiency in theory and/or high parallelism in practice, and suffer from various performance bottlenecks. We present a simple, work-efficient parallel framework for $k$-core decomposition that is easy to implement and adaptable to various strategies for improving work-efficiency. We introduce two techniques to enhance parallelism: a sampling scheme to reduce contention on high-degree vertices, and vertical granularity control (VGC) to mitigate scheduling overhead for low-degree vertices. Furthermore, we design a hierarchical bucket structure to optimize performance for graphs with high coreness values. We evaluate our algorithm on a diverse set of real-world and synthetic graphs. Compared to state-of-the-art parallel algorithms, including ParK, PKC, and Julienne, our approach demonstrates superior performance on 23 out of 25 graphs when tested on a 96-core machine. Our algorithm shows speedups of up to 315$\times$ over ParK, 33.4$\times$ over PKC, and 52.5$\times$ over Julienne.

==> algo/pseudo_MB_algorithm.tex <==
\begin{algorithm}[h]
    \caption{ParK $k$-core Decomposition Algorithm}
    \KwIn{Graph $G = (V, E)$}
    \KwOut{Core number of each vertex}
    \SetKwFor{parForEach}{parallel\_for\_each}{do}{endfor}
    
    
    \SetKwProg{myfunc}{Function}{}{}
    \myfunc{\FMain{$(G)$}}{
        $\vname{deg}[u]\gets \text{degree}$(u)\;

        $\vname{curr} \gets \emptyset$\

        $\vname{next} \gets \emptyset$\

        $\vname{coreness} \gets \emptyset$ \tcp{output array}

        $todo \gets n$\

        $level \gets 1$\

        \While{$todo > 0$}{
            \tcp{Add all nodes of $\vname{deg}[v] = \text{level}$ to $\vname{curr}$}
            \parForEach{$v \in V$}{
                \If{$\vname{deg}[v] = \text{level}$}{
                    $\vname{curr} \gets \vname{curr} \cup \{v\}$\
                }
            }
            \While{$|\vname{curr}| > 0$}{
                $todo \gets todo - |\vname{curr}|$\

                \parForEach{$v \in \vname{curr}$}{
                    $\vname{coreness}[v] \gets \vname{deg}[v]$\

                    \parForEach{$u \in \text{Neighbors}(v)$}{
                        \If{$\vname{deg}[u] > \vname{deg}[v]$}{
                            $\vname{deg}[u] \gets \vname{deg}[u] - 1$\

                            \tcp{decrease degree of $u$ atomically}
                            \If{$\vname{deg}[u] = \text{level}$}{
                                $\vname{next} \gets \vname{next} \cup \{u\}$\

                                \tcp{add sublevel node by atomically increase index}
                            }
                        }
                    }
                }
                $\vname{cur} \gets \vname{next}$\

                $\vname{next} \gets \emptyset$\
            }
            $level \gets level + 1$\
        }
        \Return{$\vname{coreness}$}\
    }
\end{algorithm}


==> algo/pseudo_bucketing.tex <==
\begin{algorithm}[h]
    \caption{Bucketing operations}
    \KwIn{Graph $G = (V, E)$ \todo{}}
    \KwOut{Coreness of each vertex}
    \SetKwFunction{FMain}{KCore}
    \SetKwFunction{FAddToBucket}{add\_to\_bucket}
    \SetKwFunction{FProcessBucket}{solve\_bucket}
    \SetKwFunction{FProcessNeighbors}{process\_neighbors}
    \SetKwFunction{FSetSampler}{set\_sampler}
    \SetKwFunction{FCheckSampleSecurity}{check\_sample\_security}
    \SetKwFunction{FCountVertex}{count\_vertex}
    \SetKwFunction{FMapNeighborsParallel}{map\_neighbors\_parallel}
    \SetKwFunction{FMapNeighborsSequential}{map\_neighbors\_sequential}
    \SetKwFunction{FFetchAndAddVertex}{fetch\_and\_add\_vertex}
    \SetKwFunction{FSampleVertex}{sample\_vertex}
    \SetKwFor{parFor}{ParallelFor}{do}{endfor}
    

    \Fn{\FAddToBucket{$u, d, base\_k$}}{
        \If{$d < base\_k$ \textbf{or} $d > (base\_k | (stride - 1))$}{
          \Return\;
        }
        \If{$d < base\_k + num\_single\_buckets$}{
          Add $u$ to single bucket\;
        }
        \Else{
          Add $u$ to intermediate buckets\;
        }
      }
      \
      
      \Fn{\FProcessBucket{$k, base\_k, offset\_k$}}{
        \tcp{Pack and add vertices from intermediate buckets to single buckets}
        $size \gets \Call{pack\_into\_pred}$ \\
        \While{$size > 0$}{
          $counting\_flag \gets \text{false}$ \\
          \parFor{$f \in frontier[0:size]$}{
            $alive[f] \gets \text{false}$ \\
            \If{$max\_core < coreness[f]$}{
                $max\_core \gets coreness[f]$ \\
            }
            \FProcessNeighbors{} \\
          }
          \If{$counting\_flag$}{
            \FCountVertex{} \\
            \tcp{Count vertices in $counting\_bag$}
          }
          $size \gets \Call{pack\_into\_pred}$ \\
        }
      }
      

==> algo/pseudo_solve.tex <==
\begin{algorithm}[h]
\caption{}
\KwIn{Vertices subset $V_{\frontier}$ in the frontier}
\SetKwFor{parFor}{parallel\_for}{do}{endfor}

\SetKwProg{myfunc}{Function}{}{}
\myfunc{\FProcessBucket{$(V_{\frontier})$}}{

  \parFor{$j \gets 0$ \textbf{to} $size - 1$}{
    $v \gets \frontier[j]$\
    
    $\alive[v] \gets \textsc{false}$\
    
    \parFor{$u \in Neighbors(v)$}{
      \If{$\coreness[u] > k$}{

        
        
        \If {$\samplemode[u] == \textsc{true}$}{
          \FSampleVertex{$(u, k)$}\;
        }
        \Else{
          $ret \gets$ \FFetchAndAddVertex{$u, -1$} \

          \If{$ret.suc == \textsc{true}$ \text{and} $ret.v == k + 1$}{ 
          
            \FAddToBucket{$(u, k)$}\

          }
        }
        
      }
    }
  }
}
\end{algorithm}


==> burdened-span-revision.tex <==
\begin{itemize}
  \item In \cref{sec:prelim}, we revised the definition of the computational model, and give the definition of \emph{span} in the standard work-span model. We also stated the result from the work-stealing scheduler~\cite{arora2001thread, BL98}, which explains how work and span are related to the running time on a parallel algorithm on $P$ processors. 
  \item At the end of \cref{sec:peeling}, we added a paragraph \emp{Span Analysis}, which analyzes the span of the existing algorithms, including \Julienne{}, and the plain version of our framework (without VGC). Indeed, the same analysis in \Julienne{} directly applies here.  We extend the analysis to the \emph{burdened span} for these algorithms. 
  \item At the end of \cref{sec:vgc}, we added a paragraph \emp{Burdened Span Analysis}, which analyzes the burdened span of our new algorithm with VGC, and compare it with \Julienne{}. This analysis helps justify why our algorithm may achieve better parallelism than \Julienne{} on certain graphs. We also briefly modified some texts in the description of the VGC part in \cref{sec:vgc} to match our new content on the analysis for burdened span. 
  \item In \cref{sec:exp:span}, we added a paragraph to experimentally evaluate the burdened span using CilkView. We compare the burdened span of our algorithm (with and without VGC) with the state-of-the-art implementation \Julienne{}. Results are provided in \cref{fig:burdened_span}. 
      The results in burdened span mostly matches the relative trend in running time. This suggests that our speedup over \Julienne{} mainly comes from better burdened span, which is enabled by using VGC to reduce synchronization overhead. 
      
      In the appendix of the full paper, we also put two figures side-by-side to make this point more clear: the speedup of our algorithm (with and without VGC) over \Julienne{} in \emph{burdened span} (\cref{fig:app:burdened_span}, the same as \cref{fig:burdened_span} in the main paper), and the speedup of our algorithm (with and without VGC) over \Julienne{} in \emph{running time} (\cref{fig:app:burdened_span_speedup}). 
      We note that, the information of \cref{fig:app:burdened_span_speedup} about the running time is fully covered in \cref{fig:overall}. 
      For page limit, we did not include \cref{fig:app:burdened_span_speedup} in the main paper, but only provide it in the full version for better illustration. 
\end{itemize}


==> figures/fig-bucketing_eg.tex <==
\begin{figure}[htbp!]
  \centering
  \includegraphics[width=\columnwidth]{figures/eg-fixed_buckets.pdf}
  \caption{\textbf{An illustration of bucketing structure.}}\label{fig:eg-bucketing}
\end{figure}


==> figures/fig-grid.tex <==
\begin{figure}[h]
  \centering
  \vspace{1em}
  \includegraphics[width=\columnwidth]{figures/eg-grid.pdf}
  \vspace{1em}
  \caption{\textbf{An $r \times r$ grid graph}}\label{fig:grid_eg}
\end{figure}

==> figures/fig-hashbag.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figures/hashbag.pdf}
  \caption{\textbf{An illustration of parallel hash bag.}}\label{fig:hashbag}
\end{figure}

==> figures/fig-illustration_combine.tex <==

\begin{figure*}[h]
  \centering
  \vspace{1em}

  \begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/eg-grid.pdf}
    \vspace{0.3em}
    \caption{\textbf{An $r \times r$ grid graph with subrounds $r/2$}}
    \label{fig:grid_eg}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/k-core-eg.pdf}
    \vspace{0.5em}
    \caption{\textbf{An illustration of one $k$-core decomposition step}}
    \label{fig:kcore_eg}
  \end{subfigure}

  % \hfill
  % \begin{subfigure}{0.36\textwidth}
  %   \centering
  %   \includegraphics[width=\textwidth]{figures/hashbag.pdf}
  %   \caption{\textbf{An illustration of parallel hash bag.}}\label{fig:hashbag}
  % \end{subfigure}
  %   \vspace{1em}
  \caption{\textbf{Combined illustration of (a) an $r \times r$ gird graph (b) VGC for an $r \times r$ grid graph.}}
  \label{fig:combined}
\end{figure*}

==> figures/fig-overall_heat.tex <==
\afterpage{
  \begin{figure}[!t]
  \centering
  \includegraphics[width=\columnwidth]{tables/speedup_transpose_heatmap.pdf}
  \caption{\textbf{Speedup Compared to \ParK, \PKC and \GBBS}}\label{fig:overall_heat}
\end{figure}
}

==> figures/fig-queue-rho.tex <==
\afterpage{
  \begin{figure*}[!h]
  \centering
  \includegraphics[width=\textwidth]{figures/charts/subrounds.pdf}
  \caption{\textbf{Decrease Ratio of $\rho$ with Local Search.} The y-axis shows the initial number of total rounds, x-axis shows the number of total rounds with local search }\label{fig:queue-rho}
\end{figure*}
}

==> related.tex <==
\section{Related Work}
The $k$-core decomposition problem has been extensively studied in various settings since it was first introduced by Seidman~\cite{seidman1983network}.
The first sequential algorithm for exact $k$-core decomposition was proposed by Matula and Beck~\cite{matula1983smallest},
using a bucket sort to arrange vertices by degree and iteratively deleting vertices with degree $k$ (peeling) until all are removed.
The algorithm runs in $O(m + n)$.
Batagelj and Zaversnik (\BZ) provided a sequential implementation that also runs within the same time complexity~\cite{batagelj2003m}. 

Several shared-memory parallel and distributed computing frameworks support $k$-core decomposition as part of graph analytics,
including GraphX~\cite{gonzalez2014graphx}, Powergraph~\cite{gonzalez2012powergraph}, Ligra~\cite{shun2013ligra} and Julienne~\cite{dhulipala2017} (later integrated into the GBBS library~\cite{gbbs2021}).
While these frameworks provide primitives for parallel or distributed graph processing, 
they do not specifically optimize for the \kcore{} problem.

There also exist studies specifically focusing on parallel \kcore{} algorithm. 
\ParK~\cite{dasari2014park} and \PKC~\cite{kabir2017parallel} are two state-of-the-art parallel algorithms using the online peeling process. 
They both use $O(n \maxcoreness + m)$ work. 
We introduced both of them in \cref{sec:peeling}. 
\PKC{} introduces optimizations, such as packing the remaining vertices after 98\% have been peeled, 
and using a local buffer to avoid subrounds.
While \PKC{} performs well on sparse graphs, 
both \Park{} and \PKC{} suffer from poor performance on dense graphs due to work-inefficiency and contention in updating induced degrees.

Dhulipala et al.~\cite{dhulipala2017} proposed a parallel \kcore{} algorithm in the \Julienne{} paper. 
In their paper, they use a bucketing structure that that maps each value $d$ to all vertices with induced degree $d$.
They proved that this algorithm has $O(m+n)$ work. In their implementation, they used a simplified bucketing structure that only 
maintains up to $b$ buckets. Our analysis proves the work-efficiency of their implementation, 
and an even simpler version without bucketing structure is also work-efficient. 
% Their algorithm is base on the offline peeling algorithm, 
\Julienne{} is based on the offline peeling approach, 
as we introduced in \cref{sec:peeling},
which is fully synchronized and race-free. 
It performs well on dense graphs but has unsatisfactory performance on sparse graphs, 
where synchronization overhead can be comparable to the computation cost.

\kcore{} is closely related to many other graph processing problems,
such as $D$-core decomposition, which extends $k$-core to directed graphs.
Several studies have explored $D$-core decomposition in both sequential and parallel/distributed settings~\cite{luo2024efficient, liao2022distributed, giatsidis2013d}.
There are also numerous approaches for approximate $k$-core decomposition, both in sequential settings~\cite{king2022computing} 
and parallel settings~\cite{esfandiari2018parallel,liu2022parallel, liu2024parallel, dhulipala2022differential}.
Additionally, streaming algorithms have been proposed for incremental $k$-core decomposition~\cite{sariyuce2013streaming, esfandiari2018parallel, sariyuce2016incremental}.















% For example, $D$-core decomposition extends $k$-core decomposition to directed graphs.
% There are some work on $D$-core decomposition both in sequential and parallel or distributed settings~\cite{luo2024efficient, liao2022distributed, giatsidis2013d}. 
%Specifically, the $D$-core decomposition problem can be reduced to the $k$-core decomposition problem when applied to undirected graphs.
%Similar to \PKC~\cite{kabir2017parallel}, their approach utilizes the same peeling process and buffer optimizations. 
%However, their algorithm is optimized for directed graphs, leading to suboptimal performance on undirected graphs.
% Thus, in this paper, we consider the exact $k$-core decomposition problem setting and related work. 










% Their algorithm initially arranges vertices by degree using a bucket sort process, 
% then iteratively deletes vertices whose degree matches the current level $k$ (peeling),
% until all vertices are removed.

%As real-world graphs have grown to billion-node scales, improving the efficiency of $k$-core decomposition algorithms has become increasingly important.
%They provide a set of primitives for parallel or distributed graph processing and solving graph problems in a more general context. 
% Most of them are graph processing frameworks which include \kcore{} as a problem in the library, and do not specifically optimize the \kcore{} problem. 
%\kcore decomposition can be solved using these frameworks, but they are not optimized for the $k$-core decomposition problem specifically.

%While the BZ algorithm is a sequential algorithm for $k$-core decomposition with a time complexity of $O(m + n)$,
%While the best sequential time complexity for \kcore{} is $O(m+n)$, 
%most existing parallel algorithms following the peeling process require $O(n \maxcoreness + m)$ work. 


%\PKC reduces the number of \subround by introducing a buffer optimization,
%but still requires $O(n \maxcoreness + m)$ work.
% \PKC{} further employs several optimizations, including packing the remaining vertices after $98\%$ of the total vertices are peeled, 
% and a local buffer that avoids subrounds in each round.  %does not significantly reduce the overall work.
% In our experiments, \PKC{} performs well on sparse graphs due to the optimizations. 
% However, on dense graphs, both \Park{} and \PKC{} may suffer from poor performance due to work-inefficiency 
% and contention in updating induced degrees concurrently.

% which is fully synchronized and is race-free. 
% In our experiments, \Julienne{} performs well on dense graphs due to race-freedom. 
% However, on sparse graphs where synchronize overhead can be comparable to the computation cost, 
% they may have unsatisfactory performance. 

% using a bucketing structure and the offline peeling framework , and Julienne~\cite{dhulipala2017}

% \input{algo/pseudo_MB_algorithm}
% Luo et al.~\cite{luo2024efficient} presented a parallel algorithm for $D$-core decomposition, 


==> tables/graph_info_full.tex <==
% Table generated by Excel2LaTeX from sheet 'graph-full'
\begin{table*}[htbp]
    \centering
  \small
        % Table generated by Excel2LaTeX from sheet 'Graph_Information'
        \begin{tabular}{rlrrrrl}
        \multicolumn{1}{l}{Category} & Name  & \multicolumn{1}{l}{n} & \multicolumn{1}{l}{m} & \multicolumn{1}{l}{C} & \multicolumn{1}{l}{$\rho$} & Notes \\
        \midrule
        \midrule
        \multicolumn{1}{l}{Social} & \LJ    & 4847571 & 85702474 & 372   & 3480  & soc-LiveJournal1~\cite{backstrom2006group} \\
              & FB    & 59216214 & 185044024 & 16    & 465   & socfb-konect~\cite{nr,traud2012social,red2011comparing} \\
              & OK    & 3072627 & 234370166 & 253   & 5667  & com-orkut~\cite{yang2015defining} \\
              & WB    & 58655849 & 522642066 & 193   & 2910  & Sina Weibo network ~\cite{nr} \\
              & TW    & 41652231 & 2405026092 & 2488  & 14964 & Twitter~\cite{kwak2010twitter} \\
              & FS    & 65608366 & 3612134270 & 304   & 10034 & Friendster~\cite{yang2015defining} \\
        \midrule
        \multicolumn{1}{l}{Web} & WK    & 6625370 & 300331770 & 188   & 3276  & enwiki-2023~\cite{BoVWFI,Boldi-2011-layered} \\
              & EH    & 11264052 & 521886106 & 9877  & 7393  & eu-2015-host~\cite{webgraph} \\
              & SD    & 89247739 & 3880015728 & 10507 & 19063 & sd-arc~\cite{webgraph} \\
              & CW    & 978408098 & 7.4744E+10 & 4244  & 106819 & ClueWeb~\cite{webgraph} \\
              & HL14  & 1724573718 & 1.24E+11 & 4160  & 58737 & Hyperlink14~\cite{webgraph} \\
              & HL12  & 3563602789 & 2.26E+11 & 10565 & 130737 & Hyperlink12~\cite{webgraph} \\
        \midrule
        \multicolumn{1}{l}{Road} & AF    & 33493259 & 88929770 & 3     & 189   & Open Street Map (OSM) Africa~\cite{roadgraph} \\
              & NA    & 86951513 & 220285922 & 4     & 286   & Open Street Map (OSM) North America~\cite{roadgraph} \\
              & AS    & 95735401 & 243624688 & 4     & 343   & Open Street Map (OSM) Asia~\cite{roadgraph} \\
              & EU    & 130655972 & 332587928 & 4     & 513   & Open Street Map (OSM) Europe~\cite{roadgraph} \\
        \midrule
        \multicolumn{1}{l}{kNN} & CH5   & 4208261 & 29650038 & 5     & 7     & Chem~\cite{fonollosa2015reservoir,wang2021geograph}, $k=5$ \\
              & GL5   & 24876978 & 157442032 & 5     & 42    & GeoLife~\cite{geolife,wang2021geograph}, $k=5$ \\
              & GL10  & 24876978 & 309743322 & 10    & 16    & GeoLife~\cite{geolife,wang2021geograph}, $k=10$ \\
              & COS5  & 321065547 & 1957750718 & 2     & 23    & Cosmo50~\cite{cosmo50,wang2021geograph}, $k=5$ \\
        \midrule
        \multicolumn{1}{l}{Synthetic} & TRCE  & 16002413 & 47997626 & 2     & 1839  & Huge traces~\cite{nr} \\
              & BBL   & 21198119 & 63580358 & 2     & 1915  & Huge bubbles~\cite{nr} \\
              & GRD   & 100000000 & 399798000 & 2     & 50499 & Huge grids~\cite{nr} \\
              & CBC   & 1000000000 & 4293239416 & 3     & 2895  & Huge cubic~\cite{nr} \\
              & HCNS  & 400000 & 3.4742E+10 & 58916 & 61888 & Huge Coreness ~\cite{nr} \\
              & HPL   & 99954272 & 1200000000 & 3980  & 6297  & Huge scale-free ~\cite{nr} \\
        \bottomrule
        \end{tabular}%

    
    %
    \vspace{1em}
      \caption{\textbf{Information of all tested graphs.} 
      $n$: \#vertices.
      $m$: \#edges in the undirected or symmetrized graph. 
      $D$: diameter of the undirected or symmetrized graph. 
      $C$: maximum coreness value.
      $\rho$: \# peeling rounds in the $k$-core decomposition.
      Undirected graphs are underlined.
      }
  \end{table*}%

